Sereum: Protecting Existing Smart Contracts Against Re-Entrancy Attacks

Recently, a number of existing blockchain systems have witnessed major bugs and vulnerabilities within smart contracts. Although the literature features a number of proposals for securing smart contracts, these proposals mostly focus on proving the correctness or absence of a certain type of vulnerability within a contract, but cannot protect deployed (legacy) contracts from being exploited. In this paper, we address this problem in the context of re-entrancy exploits and propose a novel smart contract security technology, dubbed Sereum (Secure Ethereum), which protects existing, deployed contracts against re-entrancy attacks in a backwards compatible way based on run-time monitoring and validation. Sereum does neither require any modification nor any semantic knowledge of existing contracts. By means of implementation and evaluation using the Ethereum blockchain, we show that Sereum covers the actual execution flow of a smart contract to accurately detect and prevent attacks with a false positive rate as small as 0.06% and with negligible run-time overhead. As a by-product, we develop three advanced re-entrancy attacks to demonstrate the limitations of existing offline vulnerability analysis tools.

==> acronyms.tex <==
%! TEX root = ./main.tex

\DeclareAcronym{PoC}{
  short = PoC,
  long = proof of concept
}
\DeclareAcronym{mac}{
  short = MAC,
  long = message authentication code
}
\DeclareAcronym{rop}{
  short = ROP,
  long = return-oriented programming
}
\DeclareAcronym{dop}{
  short = DOP,
  long = data-oriented programming
}
\DeclareAcronym{toctou}{
  short = TOCTOU,
  long = time-of-check vs. time-of-use
}
\DeclareAcronym{CVE}{
  short = CVE,
  long = common vulnerabilities and exposures
}
\DeclareAcronym{iot}{
  short = IoT,
  long = Internet of things
}
\DeclareAcronym{cfi}{
  short = CFI,
  long = control-flow integrity
}
\DeclareAcronym{cfg}{
  short = CFG,
  long = control-flow graph
}
\DeclareAcronym{api} {
  short = API,
  long = application programming interface
}
\DeclareAcronym{ssa} {
  short = SSA,
  long = single static assignment
}
%\DeclareAcronym{URL} {
%  short = URL,
%  long = uniform resource locator
%}
\DeclareAcronym{CPU} {
  short = CPU,
  long = central processing unit
}
\DeclareAcronym{vtable} {
  short = vtable,
  long = virtual method table
}
\DeclareAcronym{OS} {
  short = OS,
  long = operating system
}

\DeclareAcronym{evm} {
  short = EVM,
  long = Ethereum virtual machine
}

\DeclareAcronym{rpc} {
  short = RPC,
  long = remote procedure call
}
\DeclareAcronym{aDAO}{
  short = DAO,
  long = distributed autonomous organization
}
\DeclareAcronym{tee}{
  short = TEE,
  long = trusted execution environment,
}


==> figures/fig_common.tex <==
\usepackage[utf8]{inputenc}
\usepackage[english]{babel}
\usepackage[T1]{fontenc}
\usepackage{lmodern}

\usepackage{times}

\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{amsfonts}
\usepackage{amsfonts}
\usepackage{amsthm}

\usetikzlibrary{shapes,arrows,positioning,shapes.multipart}
\usetikzlibrary{backgrounds}
\usetikzlibrary{fit}
\usetikzlibrary{calc}
\usetikzlibrary{trees}
\usetikzlibrary{calc}
\usetikzlibrary{matrix}

\input{../lstconfig}
\input{../circled}
\input{../macros}



==> figures/performance-table.tex <==
\begin{tabular}{l r r}
  \toprule
  Type        & Mean & $\sigma$ \\
  \midrule
  \emph{geth} & 2277.0 ms & 146.7 ms \\
  \toolname   & 2494.5 ms & 174.8 ms \\
  Overhead    & 217.6 ms  & 100.9 ms \\
  \bottomrule
\end{tabular}


==> figures/taintprop-as-table.tex <==
\tikzstyle{freecell}=[fill=white]

\begin{tabularx}{\linewidth}{r c p{5cm} p{5cm} p{5cm}}
PC &%%
Instruction &%%
Stack (before Instruction) &%%
Shadow Stack (Taints) &%%
Taint Engine \\%
1 &%%
\texttt{SLOAD} &%%
\begin{drawstackc}
  \cell{$A$} \cellptr{top}
  \cell{$C$}
  \stackbottom
\end{drawstackc} &%%
\begin{drawstackc}
  \cell{$\tau_{\emptyset}$} \cellptr{top}
  \cell{$\tau'$}
  \stackbottom
\end{drawstackc}
 &%
Create new \emph{DependsOnStorage} taint $\tau_S$ associated with address $A$ and push
  it onto the shadow stack. \\
2 &%
\texttt{LT} &%
\begin{drawstackc}
  \cell{$V$} \cellptr{top}
  \cell{$C$}
  \stackbottom
\end{drawstackc}
 &%
\begin{drawstackc}
  \cell{$\tau_S$} \cellptr{top}
  \cell{$\tau'$}
  \stackbottom
\end{drawstackc}
 &%
Take the taints of the two instruction operands, $\tau_S$ and
$\tau'$ and assign both to $b$ by moving them to the same stack slot. \\
3 &%
\texttt{PUSH2 dst} &%
\begin{drawstackc}
  \cell{}
  \cell{$b = V < C$} \cellptr{top}
  \stackbottom
\end{drawstackc}
&%
\begin{drawstackc}
  \cell{}
  \cell{ $\tau_S, \tau'$ } \cellptr{top}
  \stackbottom
\end{drawstackc}
 &%
Push empty taint for constant \texttt{dst}.\\
4 &%
\texttt{JUMPI}&%
\begin{drawstackc}
  \cell{ \texttt{dst} } \cellptr{top}
  \cell{ $b = V < C$ }
  \stackbottom
\end{drawstackc}
&%
\begin{drawstackc}
  \cell{ $ \tau_{\emptyset} $ } \cellptr{top}
  \cell{ $\tau_S, \tau'$ }
  \stackbottom
\end{drawstackc}
&%
Check the taints of the jump condition: If it is tainted with a
\emph{DependsOnStorage} taint ($\tau_S$), then compute original address $A$
from taint and record that the variable at storage address $A$ influenced
control-flow. \\
\end{tabularx}


==> sections/discussion.tex <==
%! TEX root = ../main.tex

Due to time constraints, we did evaluate \toolname\ only on a subset of the
Ethereum blockchain. As future work we plan to run \toolname\ on the rest of
the blockchain, further searching for re-entrancy attacks. 

